Towards Backdoor Attacks and Defense in Robust Machine Learning Models

The introduction of robust optimisation has pushed the state-of-the-art in defending against adversarial attacks. Notably, the state-of-the-art projected gradient descent (PGD)-based training method has been shown to be universally and reliably effective in defending against adversarial inputs. This robustness approach uses PGD as a reliable and universal "first-order adversary". However, the behaviour of such optimisation has not been studied in the light of a fundamentally different class of attacks called backdoors. In this paper, we study how to inject and defend against backdoor attacks for robust models trained using PGD-based robust optimisation. We demonstrate that these models are susceptible to backdoor attacks. Subsequently, we observe that backdoors are reflected in the feature representation of such models. Then, this observation is leveraged to detect such backdoor-infected models via a detection technique called AEGIS. Specifically, given a robust Deep Neural Network (DNN) that is trained using PGD-based first-order adversarial training approach, AEGIS uses feature clustering to effectively detect whether such DNNs are backdoor-infected or clean. In our evaluation of several visible and hidden backdoor triggers on major classification tasks using CIFAR-10, MNIST and FMNIST datasets, AEGIS effectively detects PGD-trained robust DNNs infected with backdoors. AEGIS detects such backdoor-infected models with 91.6% accuracy (11 out of 12 tested models), without any false positives. Furthermore, AEGIS detects the targeted class in the backdoor-infected model with a reasonably low (11.1%) false positive rate. Our investigation reveals that salient features of adversarially robust DNNs could be promising to break the stealthy nature of backdoor attacks.

==> setup.tex <==
%\clearpage
\section{Experimental Setup}
\label{sec:setup}


\subsection{Datasets and Models}
%\todo{cite datasets, resnet}
In our evaluation, we use three major datasets, namely CIFAR-10~\cite{krizhevsky2009learning}, MNIST~\cite{lecun1998mnist} and Fashion-MNIST~\cite{xiao2017online}. MNIST and Fashion-MNIST models were trained with the standard ResNet-18 architecture, while CIFAR-10 models were trained using the standard ResNet-50 architecture~\cite{he2016deep}. All experiments were conducted with the default learning rate (LR) scheduling in the robustness package~\cite{robustness-lib}, i.e.   the PyTorch StepLR optimisation scheduler. The learning rate is initially set to 0.1 for training (LR) and the scheduler decays the learning rate of each parameter group by 0.1 (gamma) every 50 epochs (default step size). All models were trained with momentum of 0.9 and weight decay of $5e^{-4}$. Only CIFAR-10 models were trained with data augmentation, this is the default configuration in the robustness package for CIFAR-10.

\begin{table*}[h]
  \begin{center}
  %\vspace*{-0.1in}
  {%\scriptsize
  \begin{tabular}{|l|r|r|r|r|} %r|r|}
    \hline 
\multicolumn{1}{|c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\multirow{1}{*}{\textbf{Epochs}}} & \multicolumn{1}{c|}{\textbf{LR}} & \multicolumn{1}{c|}{\textbf{Batch Size}}  & \multicolumn{1}{c|}{\textbf{LR Schedule}} \\ 
%          \multicolumn{1}{|c|}{\textbf{Type}} & \multicolumn{1}{c|}{(\#labels)}  & & \multicolumn{1}{c|}{\textbf{Size}} & \multicolumn{1}{c|}{\textbf{training}} & \multicolumn{1}{c|}{\textbf{test}} \\ 
    \hline
     CIFAR-10  & 110  &  0.1 & 128 & Drop by 10 at epochs  $\in [50, 100]$ \\  
    \hline	
    MNIST  & 100  & 0.1 & 128 & Drop by 10 at epochs  $\in [50, 100]$  \\ 
    \hline
    Fashion-MNIST & 100  & 0.1 & 128 & Drop by 10 at epochs  $\in [50, 100]$  \\  
     \hline     
    \end{tabular}}
    \caption{Standard Hyperparameters used for model training.}
  \label{tab:hyperparameters}   
\end{center}
\end{table*}


\subsection{Adversarial Training}
For our evaluation, all models were trained with robust optimisation based on the adversarial training approach of~\cite{pgd-madry} with an $l_2$ perturbation set. The parameters for robust training are the same for all datasets. In particular, all models were trained with an adversarial attack budget of $0.5$ ($\epsilon$), and an attack step size of $1.5$ (step size) and set to take $20$ steps (\# steps) during adversarial attack (\textit{cf. \Cref{tab:adv-training}}). All other hyperparameters are set to the default hyperparameters (\textit{cf. \Cref{tab:adv-training}}) in the robustness package~\cite{robustness-lib}. No hyperparameter tuning was performed for the adversarial training of models. 

\begin{table}[h]
  \begin{center}
  %\vspace*{-0.1in}
  {%\scriptsize
  \begin{tabular}{|l|r|r|r|} %r|r|}
    \hline 
\multicolumn{1}{|c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\multirow{1}{*}{\textbf{$\epsilon$}}} & \multicolumn{1}{c|}{\textbf{\# steps}} & \multicolumn{1}{c|}{\textbf{Step size}}  \\ 
    \hline
     CIFAR-10  &  0.5  & 20 & 1.5  \\  
    \hline	
    MNIST  &  0.5  & 20 & 1.5   \\ 
    \hline
    Fashion-MNIST &  0.5  & 20 & 1.5   \\  
     \hline     
    \end{tabular}}
    \caption{Hyperparameters used for adversarially robust model training and evaluation.}
  \label{tab:adv-training}   
\end{center}
\end{table}
 
%\subsection{Hyperparameter Tuning}
%\clearpage
\subsection{Adversarial Accuracy}
%
%\begin{table}[h]
%  \begin{center}
%  %\vspace*{-0.1in}
%  {%\scriptsize
%  \begin{tabular}{|l|r|r|r|} %r|r|}
%    \hline 
%\multicolumn{1}{|c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\multirow{1}{*}{\textbf{$\epsilon$}}} & \multicolumn{1}{c|}{\textbf{\# steps}} & \multicolumn{1}{c|}{\textbf{Step size}}  \\ 
%    \hline
%     CIFAR-10  &  0.5  & 20 & 0.1  \\  
%    \hline	
%    MNIST  &  0.5  & 20 & 0.1   \\ 
%    \hline
%    Fashion-MNIST &  0.5  & 20 & 0.1   \\  
%     \hline     
%    \end{tabular}}
%    \caption{Hyperparameters used for adversarially robust model evaluation.}
%  \label{tab:adv-evaluation}   
%\end{center}
%\end{table}

Adversarial evaluation was performed with the same parameters as adversarial training for all datasets and models. In particular, all classifiers were evaluated with an adversarial attack budget of $0.5$ ($\epsilon$), and an attack step size of $1.5$ and set to take $20$ steps during adversarial attack (\textit{cf. \Cref{tab:adv-training}}). In addition, for adversarial evaluation, we use the best loss in PGD step as the attack ('use\_best': True,), with no random restarts ('random\_restarts': 0) and no fade in epsilon along epochs ('eps\_fadein\_epochs': 0). Overall, results showed that all models maintained a similarly high adversarial accuracy for both clean and backdoor-infected models (\textit{cf. \Cref{tab:adv-accuracy}}). Specficially, 86.22\%  adversarial accuracy, on average. Hence, adversarial training accuracy is not inhibited by the backdoor attack vector.


\begin{table}[h]
  \begin{center}
  %\vspace*{-0.1in}
  {%\scriptsize
  %\footnotesize
  \begin{tabular}{lr|r|r|r|}
	\hline  
	\multicolumn{1}{|c|}{\multirow{4}{*}{\shortstack{\textbf{Dataset}}} }& \multicolumn{3}{c|}{\textbf{Adversarial Accuracy}} \\ %& \multirow{4}{*}{\shortstack{\textbf{Clean}\\\textbf{Model}}}  \\
	\multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{\textbf{Backdoor-Infected Models}}  & \multirow{2}{*}{\shortstack{\textbf{Clean}\\\textbf{Model}}} \\
	%&   & \\
	\multicolumn{1}{|c|}{} & \textbf{Localised} & \textbf{Distributed}  &  \\
	\hline
	\multicolumn{1}{|c|}{CIFAR-10} & 68.26 & 68.17 & 68.64  \\  
    \hline    
  	\multicolumn{1}{|c|}{MNIST} & 99.51 & 99.49 & 99.55 \\
	\hline  
	\multicolumn{1}{|c|}{Fashion-MNIST} &90.78 & 90.66 & 90.91 \\
    \hline     
    \end{tabular}}
  \caption{Adversarial accuracy of all robust classifiers.}
  \label{tab:adv-accuracy}   
  \vspace*{-0.2in}
\end{center}
\end{table}




%\subsection{Image translation}
%
%\begin{table}[h]
%  \begin{center}
%  %\vspace*{-0.1in}
%  {%\scriptsize
%  \begin{tabular}{|l|r|r|r|} %r|r|}
%    \hline 
%\multicolumn{1}{|c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\multirow{1}{*}{\textbf{$\epsilon$}}} & \multicolumn{1}{c|}{\textbf{\# steps}} & \multicolumn{1}{c|}{\textbf{Step size}}  \\ 
%    \hline
%     CIFAR-10  &  X  & X & X  \\  
%    \hline	
%    MNIST  &  X  & X & X  \\ 
%    \hline
%    Fashion-MNIST &  X  & X & X   \\  
%     \hline     
%    \end{tabular}}
%    \caption{Parameters used for image translation.}
%  \label{tab:adv-training}   
%\end{center}
%\end{table}
%
%\subsection{Detection Parameters}



==> training_desc.tex <==
\section{Training Description}
In the standard training of machine learning models, loss functions are 
generally based on the concept of Empirical risk minimisation (ERM). The core 
idea is that we cannot know exactly how well an algorithm will work in practice 
(the true "risk") because we don't know the true distribution of data that the 
algorithm will work on, but we can instead measure its performance on a known 
set of training data (the "empirical" risk). However, ERM based loss functions 
produce models that are not robust to adversarial examples. 
Formally, ERM based models want to minimise:

\begin{equation}
%f = \min_{f} 
\mathbb{E}_{x \sim \mathcal{D}} 
\left[\mathcal{L}(x, y^{(i)})\right]
\label{eqn:erm_training}
\end{equation}

Here $x$ and $y^{(i)}$ are the input and the and ground truth value of this 
input respectively and $\mathcal{L}$ is a loss function.



In order to reliably train models against these attacks, robust optimisation 
formally specifies a set of allowed perturbations $\Delta$ (Usually an $L_2$ or 
$L_{\infty}$ ball around the input) and modifies the classic ERM loss function 
to minimise the maximum loss in this region, giving rise to the
min-max optimisation used in robust optimisation. Intuitively, it is useful to 
think of each input $x$ as having a region $\Delta$ 
around the vicinity associated with 
it. The robust optimisation tries to ensure that the region region $\Delta$
has the same output as the ground truth of the value $y^{(i)}$. 
Formally robust optimisation wants to minimise:
\begin{equation}
%f = \min_{f} 
\mathbb{E}_{x \sim \mathcal{D}} 
\left[\max_{\delta \in \Delta} \mathcal{L}(x+\delta, y^{(i)})\right]
\label{eqn:robust_training}
\end{equation}

